Neutrino Scattering: Connections Across Theory and Experiment

In this document drafted by the Neutrino Scattering Theory Experiment Collaboration (NuSTEC), we provide input on the synergies between theoretical and experimental efforts that can provide critical input to the prediction accuracy needed for the forthcoming high-precision neutrino measurements. These efforts involve a wide range of energies and interaction processes, as well as target nuclei and interaction probes. The challenges discussed will be overcome only through the active support of integrated collaboration across strong and electroweak physics from both the nuclear and high energy physics communities.

==> authors.tex <==
\author{L.~Alvarez-Ruso}\affiliation{\IFIC}
\author{A.M. Ankowski}\affiliation{\Wroclaw}
\author{A.~Ashkenazi}\affiliation{\TAU}
\author{M.~Betancourt}\affiliation{\FNAL}
\author{M.~Sajjad Athar}\affiliation{\Aligarh}
%\author{M.B.~Barbaro}\affiliation{\Torino}
%\author{A.~De Roeck}\affiliation{\CERN}
%\author{S.~Dolan}\affiliation{\CERN}
\author{E.~Catano-Mur} \affiliation{\WandM}
\author{P.~Coloma}\affiliation{\IFT}
\author{P.~Dunne}\affiliation{\Imperial}
\author{L.~Doria}\affiliation{\Mainz}
%\author{K.E.~Duffy}\affiliation{\Oxford}
\author{A.~Garcia-Soto}\affiliation{\IFIC}
\author{S.~Gardiner}\affiliation{\FNAL}
\author{R.~Gonz\'alez-Jim\'enez}\affiliation{\Sevilla}
%\author{R.~Gran}\affiliation{\Duluth}
\author{P.~Huber}\affiliation{\CNP}
%\author{N.~Jachowicz}\thanks{Contact person}\affiliation{\Ghent}
%\author{T.~Katori}\affiliation{\London}
%\author{A.S.~Kronfeld}\affiliation{\FNAL}
\author{E.~Kajomovitz Ken}\affiliation{\Technion}
%\author{X.-G.~Lu}\affiliation{\Warwick}
\author{J.~Kopp}\affiliation{\CERN}\affiliation{\Mainza}
\author{I. Martinez-Soler}\affiliation{\IPPP}
%\author{K.~Mahn}\affiliation{\Michigan}
\author{A.~S.~Meyer}\affiliation{\LLNL}
\author{L.~Munteanu}\affiliation{\CERN}
\author{A.~Nikolakopoulos}\affiliation{\INT}
\author{V.~Pandey}\affiliation{\FNAL}
\author{A.~Papadopoulou}\affiliation{\Argonne}
%\author{S.~Pastore}\affiliation{\StLouis}
%\author{I. Ruiz Simo}\affiliation{\Granada}
%\author{F.~S\'anchez}\affiliation{\Geneva}
\author{M.~Scott}\affiliation{\Imperial}
%\author{J.T.~Sobczyk}\affiliation{\Wroclaw}
\author{N.~Rocco}\affiliation{\FNAL}
\author{J.E.~Sobczyk}\affiliation{\Mainz}
%\author{M.~Cristina Volpe}\affiliation{\CNRS}
%\author{A.~Weber}\affiliation{\Mainza}\affiliation{\FNAL}
\author{C.~Wret}\affiliation{\Imperial}
\author{Z.~Tabrizi}\affiliation{\Pittsburgh}\affiliation{\CERN}

==> exp_IceCube.tex <==
\textit{Anatoli Fedynitch}

The IceCube Neutrino Observatory, located at the South Pole, instruments a cubic kilometer of ice with 5160 digital optical modules — each housing a 10" photomultiplier tube — arranged along 86 vertical strings. 
Its central DeepCore subarray lowers the energy threshold to capture atmospheric neutrinos above 5 GeV for studies of neutrino properties, interactions, and physics beyond the Standard Model, while the remaining 78 strings, optimized for a threshold near 100 GeV, target cosmic-ray and astrophysical neutrino sources.

Advances in detector modeling~\cite{IceCubeCollaboration:2023wtb} and machine learning event reconstruction have enabled IceCube to achieve leading measurements of the oscillation parameters $\theta_{23}$ and $\Delta m^{2}_{32}$ via the $\nu_\mu$ disappearance channel using only atmospheric neutrinos \cite{PhysRevLett.134.091801}. 
It has also evaluated PMNS matrix unitarity by measuring $\nu_\tau$ appearance~\cite{IceCube:2019dqi}, and its broad energy coverage supports diverse tests of non-standard neutrino interactions and phenomena beyond the Standard Model \cite{IceCubeCollaboration:2024nle}.

IceCube further probes neutrino interactions directly by analyzing the inelasticity distribution in the $50\,\text{GeV} < E_\nu < 560\,\text{GeV}$ range \cite{IceCube:2025tvs} and at TeV energies~\cite{IceCube:2018pgc}, and by determining cross sections through the absorption of atmospheric neutrinos traversing Earth~\cite{PhysRevD.104.022001}. 
The identification of flavor from interactions of astrophysical neutrinos benefits from future improvements in modeling accuracy of neutrino interactions at TeV and PeV, as exemplified by the detection of a Glashow Resonance event near 6.3 PeV \cite{IceCube:2021rpz} — a direct probe of astrophysical neutrino flavor composition — and by tests of quantum gravity~\cite{ICECUBE:2023gdv}.  
These results complement efforts by~\textit{FASER} at the LHC and will benefit from the planned~\textit{Forward Physics Facility}.

Scheduled to begin data taking in 2026, the IceCube Upgrade is the first step toward the larger IceCube-Gen2 project. 
This phase will add seven densely instrumented strings within DeepCore, lowering the detection threshold into the GeV range and reducing systematic uncertainties across all energies through dedicated calibration hardware~\cite{Yanez}. 
The upgrade aims to produce leading measurements of atmospheric neutrino oscillation parameters, achieve world-leading precision in $\nu_\tau$ appearance measurements, and significantly advance our understanding of the neutrino mass ordering.  
Because uncertainties in cross sections, detector response, and atmospheric fluxes all equally limit precision, reducing them simultaneously is essential. 
Hence, advancing our understanding of neutrino interaction physics is crucial to fully harnessing IceCube’s contributions to fundamental physics.

==> exp_KM3NET.tex <==
The KM3NeT neutrino infrastructure consists of two detectors, ORCA and ARCA~\cite{Adrian-Martinez:2016fdl}. 
ORCA is being constructed at a depth of 2,500 meters off the French coast near Toulon, while ARCA is located 3,500 meters deep near Porto Palo in Sicily. 
Both detectors use the same technology, with the primary difference being the spacing of their digital optical modules (DOMs). 
ORCA has a denser configuration, comprising 115 lines with 18 DOMs each, distributed within a volume equivalent to 8 MTon. 
In contrast, ARCA features a sparser arrangement, with 230 lines covering approximately 1 km3 of sea water. 
At the time of this writing, 24 ORCA lines and 33 ARCA lines have been deployed, with further installations planned in the coming months. 
The difference in size and density drives the physics focus of each configuration. 

ORCA is optimized for the study of atmospheric neutrinos with energies ranging from 3 GeV to several hundred GeV. 
Its primary objective is to determine the relative ordering of neutrino masses. 
This ordering affects neutrino oscillations in matter, leaving an imprint on the atmospheric neutrino flux through characteristic appearance/disappearance patterns for the different neutrino flavors as a function of energy and path through the Earth. 
Similar to HK, most of ORCA's sensitivity comes from upgoing events with energies between 5 and 10 GeV~\cite{KM3NeT:2021ozk,KM3NeT:2021rkn}. 
Therefore, precise knowledge of the atmospheric neutrino flux and neutrino-water cross section in this energy range is essential. 
Recent analyses with an initial six-line configuration have demonstrated ORCA’s immense potential not only for studying neutrino oscillations but also for probing BSM physics~\cite{KM3NeT:2024ecf,KM3NeT:2024jji,KM3NeT:2024pte,KM3NeT:2025tiq,KM3NeT:2025ftj}. 
%The event generator used to simulate neutrino interaction in these analyses is GENIE, using the tune \texttt{G18\_02a\_00\_000}. 
As more data is collected, improving our understanding of DIS and hadronization in this energy regime will become increasingly important~\cite{Seckel_1998,Alikhanov_2016,PhysRevD.101.036010,PhysRevD.101.036011,PhysRevD.111.043007}.

ARCA’s main goal is the detection of high-energy neutrinos from astrophysical sources, with energies ranging from a few TeV to PeV~\cite{KM3NeT:2024paj}. Due to its geographical location and excellent pointing accuracy, ARCA is particularly well-suited for identifying neutrino sources within the Milky Way at TeV energies. Additionally, even with a partial configuration of 21 lines, ARCA recently reported the most energetic neutrino ever observed—at 220 PeV—opening a new window to ultra-high-energy neutrino astronomy~\cite{KM3NeT:2025npi}. At energies above few tens of TeV, neutrino interactions with matter become significant in a process known as Earth attenuation, where neutrinos can interact with quarks during their passage through the Earth before reaching the detector. These deep inelastic interactions depend on nuclear properties, making it essential to accurately model nuclear effects at high energies. Currently, the event generator used for ARCA simulations is the HEDIS module of GENIE~\cite{Garcia:2020jwr}, using the tune with the CSMS model~\cite{Cooper-Sarkar:2011jtt}.


==> exp_NuSTORM.tex <==
\newcommand{\gsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{>}{\scriptstyle \sim}\;$}}}
\newcommand{\lsim}      {\mbox{\raisebox{-0.4ex}{$\;\stackrel{<}{\scriptstyle \sim}\;$}}}

Muon decay is one of the very few sources of electron neutrinos in the energy range, 0.1-10\,GeV, relevant for oscillation and long-baseline experiments. 
Muons have a sufficient lifetime to allow effective formation of pure beams. 
Therefore, the concept of storing muon beams for neutrino production has been explored in many different contexts, see {\it e.g.}~\cite{Neuffer:1983xya,Geer:1997iz,nuSTORM:2012jbd,Ahdida:2020whw}. 
Using these beams for long-baseline experiments would require very high luminosity and this in turn makes the muon production system complex and expensive. 
On the other hand, for measuring cross sections (or in general fixed-target experiments), relatively simple muon production methods can be used based on existing proton beam facilities existent at many accelerator laboratories like Fermilab and CERN. 
The storage rings for energies in the GeV range are compact as well. Beam instrumentation allows to know the neutrino flux at the percent-level and potentially much better than that. 

The opportunity to implement nuSTORM at CERN has been studied in detail~\cite{Ahdida:2020whw}.  The proposed facility is capable of storing $\mu^\pm$ beams with momentum of between 1\,GeV/c and 6\,GeV/c and a momentum spread of $\pm 16$\%. %producing neutrino beams with energies in the range 300\,MeV to 5.5\,GeV.  
This will allow neutrino-scattering measurements to be made over the kinematic range of interest to the DUNE and Hyper-K collaborations.  Synthetic neutrino beams 
%with an RMS energy spread $\sim 0.5$\,GeV 
can be created by combining neutrinos from muon beams stored at a variety of different energies~\cite{Jurj:2025nmm}.

A detector placed on the axis of the nuSTORM production straight will receive a bright flash of muon neutrinos from pion decay followed by a series of pulses of muon and electron neutrinos from subsequent turns of the muon beam.  Appropriate instrumentation in the decay ring and production straight will be capable of determining the integrated neutrino flux with a precision of $\lsim 1$\%.  The flavour composition of the neutrino beam from muon decay is known and the neutrino-energy spectrum can be calculated precisely using the Michel parameters and the optics of the muon decay ring.  The pion and muon momenta ($p_\pi$ and $p_\mu$) can be optimised to measure $\parenbar{\nu}\!\!_e A$ and $\parenbar{\nu}\!\!_\mu A$ interactions with per-cent-level precision over the neutrino-energy range $0.3 \lsim E_\nu \lsim 5.5$\,GeV and to search for light sterile 
neutrinos with excellent sensitivity. 

Once the neutrino source is known at this level, the challenge for cross section measurements then becomes to have detector systems that can match that precision, covering a large phase space efficiently and reconstructing particle properties precisely -- this is a common challenge for all neutrino sources. 
%It also presents a challenge for theory and event generators, since usually theory computes idealized event types like quasi-elastic, but detectors usually observe a mix of events summarized as quasi-elastic-like, for instance, no hadronic activity and only a leading lepton. A less ambitious approach could be to regard these precision beams as detector test beams, where smaller versions of functionally very similar detectors are exposed and their responses is recorded.

A relatively less explored idea, but considered in nuSTORM feasibility studies at CERN, is to use these neutrino precision beam facilites as laboratories for new physics searches, especially for light dark sectors~\cite{nuSTORM:2022div}.


==> exp_atmospheric_nu.tex <==
\textbf{Atmospheric neutrinos:} are produced when cosmic rays collide with atmospheric nuclei, generating mesons and muons that decay into electron and muon neutrinos~\cite{Gaisser:2002jj,Yanez:2023lsy}. At energies above the TeV scale, tau neutrinos ($\nu_{\tau}$) are produced through D meson decays~\cite{Enberg:2008te}. The atmospheric neutrino flux spans a wide energy range, from approximately $10$~MeV to $10$~TeV, beyond which astrophysical neutrinos dominate~\cite{IceCube:2013low}. The sub-GeV flux has been measured by Super-Kamiokande~\cite{Super-Kamiokande:2023ahc}, while high-energy measurements come from large detectors like IceCube~\cite{IceCube:2024xjj,Abbasi:2021qfz} and KM3NeT~\cite{KM3NeT:2024ecf}. Future experiments, including DUNE~\cite{DUNE:2020ypp} and Hyper-Kamiokande~\cite{Hyper-Kamiokande:2018ofw}, will improve measurement precision.

==> exp_eA.tex <==
An effective way to enhance our understanding of neutrino-nucleus interactions is through
electron-nucleus scattering experiments~\cite{e4nu,RevModPhys.80.189}.
Electrons share with neutrinos the vector component of the interaction with nuclei,
providing a clean and well-controlled probe of complex nuclear dynamics.
Electron beams can be precisely tuned to a well-defined energy, allowing for the
separation of different final states and enabling high-statistics experiments.
Electron-nucleus scattering can provide valuable insights into nuclear effects that
also influence neutrino interactions, namely:

\begin{itemize}

\item Nuclear Structure and Response:
Electron scattering experiments allow precise mapping of nucleon momentum distributions and nuclear densities.
This information helps refine nuclear models used in neutrino interaction simulations.

\item Final State Interactions (FSI):
After a neutrino interacts with a nucleus, the resulting particles propagate through the nuclear medium,
experiencing rescattering, absorption, or emission.
With electron scattering, FSI can be studied selecting precise final states.

\item Quasielastic scattering and pion production:
In neutrino experiments, different effects corresponding to different energy ranges
(quasielastic, resonance production, and deep-inelastic scattering) contribute to the total cross section.
Data provided by electron scattering serve as benchmarks for validating models across these regimes.

\item Neutrino Energy Reconstruction:
One of the key challenges in neutrino experiments is reconstructing the incoming neutrino energy
from the observation of particles in the final state.
Electron scattering experiments provide a test for energy reconstruction methods by comparing
measured and theoretical cross sections.
\end{itemize}

Present electron scattering facilities pursuing an electron-nucleus scattering program aimed at neutrino
physics are the Thomas Jefferson National Accelerator Facility in the USA~\cite{mariani,JLab_Inclusive,JLab_Ti,JLab_Exclusive} (up to 12~GeV beam energy)
and the MAMI facility in Germany~\cite{MAMI1,MAMI2,Mihovilovic} (up to 1.6~GeV beam energy). In the near future, more experimental efforts from other experiments are planned (LDMX~\cite{LDMX} experiment, eALBA at the ALBA synchrotron in Barcelona, Spain)
or under construction (MESA, 155~MeV energy-recovery accelerator~\cite{MESAscience} in Mainz, Germany).

\subsubsection{Muon scattering}
In a similar way to the discussion in the previous section, it is possible to use muon-nucleus scattering to enhance our understanding of the neutrino-nucleus interactions. The highly energetic muons from the LHC that interact with the tungsten in the FASER$\nu$ experiment provide us with an excellent probe to study complex nuclear dynamics for energy transfers of the order of 10s of GeVs, thus providing valuable insights into nuclear effects that also influence neutrino interactions extending the kinematic regime that is proved by the electron-scattering.

==> exp_intro.tex <==
The experimental study of neutrino oscillations spans a wide range of experiments, each designed to constrain different oscillation parameters by examining the appearance or disappearance of specific neutrino flavors across different energy regions.

All of these experiments rely on heavy nuclei as targets, meaning their accuracy is fundamentally limited by our understanding of neutrino-nucleus interactions at different energy scales.

This section provides an overview of the various experiments, organized from the lowest to the highest incoming neutrino energy range. 

To address some of the challenges in neutrino interaction modeling, the final subsection highlights dedicated experiments that aim to refine these models and reduce uncertainties using both neutrino and electron scattering data.






==> exp_nuA.tex <==
\textit{Laura Munteanu}
Future-generation neutrino experiments such as DUNE will make precision measurements of oscillation parameters and will be sensitive not only to the total number of oscillated events, but also to the evolution of the latter as a function of true neutrino energy. The use of near detectors is of paramount importance in this endeavor, but a reliable and robust cross-section model is needed in order to extrapolate the near detector constraints to the oscillated spectra. This is a requirement even when using the PRISM technique, as there are intrinsic backgrounds and phase spaces outside detector acceptances which cannot be constrained with this method and rely on the modeling of neutrino-nucleus cross sections.

The key areas which need to be addressed in preparation for the next-generation experiments' program are:
\begin{itemize}
    \item The relationship between the true and the reconstructed energy. Nuclear effects which alter the amount of visible energy in a detector can impact the shape of the oscillated spectrum in a way which is degenerate with neutrino oscillations (see e.g. \cite{}). Whereas it is inevitable that some fraction of the neutrino energy will be invisible inside the detector (i.e. there will always be a neutrino energy bias), the uncertainty on this difference must be reduced to a level compatible with the target precision on oscillation measurements. 
    \item Differences between the cross sections for different neutrino flavors and neutrinos and anti-neutrinos. Although in principle these differences are predictable thanks to the assumption of lepton universality, mass differences between neutrino flavors (notably electron and muon neutrinos) become significant in areas of the interaction phase space which have large associated uncertainties (for example, at low energy transfers, where models differ substantially in the way in which they incorporate the treatment of FSI, optical potential, Pauli blocking or long-range correlations).
    \item The energy dependence of the cross section. Due to oscillations, the flux probed by near detectors is different from the one seen at the far detector. To reliably extrapolate near detector constraints to the far detector, the evolution of the cross section must be known for the range of energies relevant for oscillation searches.
\end{itemize}

The knowledge of the relationship between the true and reconstructed neutrino energy is perhaps the most challenging of these requirements. In a liquid argon detector such as DUNE, a portion of the neutrino energy is reconstructed through visible energy deposits. However, a significant portion of the neutrino energy is transferred to particles which cannot be identified and bias the reconstructed neutrino energy. The main sources of missing energy are:
\begin{itemize}
    \item neutrons produced in neutrino interactions. Since neutrons do not ionize the liquid argon, they cannot be detected by their tracks. Although some neutrons can be reconstructed via their secondary interactions, the cross section of these processes is not well known and relies on sub-nanosecond timing resolution in order to infer the kinematics of the neutron. The main mechanisms through which neutrons are produced in neutrino interactions is through FSI. In anti-neutrino interactions, due to parity considerations, neutrons are also produced at the vertex, in addition to those produced in FSI mechanisms. 
    \item the production of charged pions. The latter deposit energy inside a detector through ionization, but it is not always possible to determine the number of pions produced in an interaction. As a result, pion production processes contribute with integer multiples of the pion mass (i.e. 139.57 MeV) to the neutrino energy bias. Charged pions are produced through resonant interaction, but also shallow and deep inelastic scatters, as well as through FSI. In practice, neutrino experiments rely on the use of Monte Carlo generators to predict these quantities, and the latter rely on numerical hadronization routines and cascade models. The lack of theoretical guidance and experimental guidance in this region means that models targeting pion production process or hadronization have poor predictive power.  
\end{itemize}

In addition to the necessary theory developments outlined in \autoref{}, it is essential to have high-quality neutrino scattering measurements in order to benchmark these mechanisms. Several experimental programs targeting them have already been proposed. For instance, the Upgraded T2K near detector will be able to measure the kinematics of neutrons produced at T2K and HK energies, thanks to its sub-nanosecond timing resolution and fine granularity. Whilst valuable, these measurements will be made on a hydrocarbon target, whereas it is also necessary to gain insight into neutron production at DUNE energies and on liquid argon. Several measurements targeting pion production processes exist from the MINERvA, T2K and MicroBooNE collaborations \cite{}, but are either on hydrocarbon or at low energies compared to DUNE's region of interest. The SBND and ICARUS experiments will provide some of the first high-statistics measurements on liquid argon, although at lower energies than those of DUNE. In addition, these experiments will become systematically limited, notably by the knowledge of the neutrino flux. Indeed, the fact that the incoming energy is not known precisely hinders the range of measurements which can be made with conventional setups.

A promising avenue for future measurements would be the construction of a dedicated experiment using monitored and tagged neutrino beams at CERN \cite{}. Such an experiment would allow for a dedicated measurement of the neutrino cross section evolution as a function of energy, as well as multi-differential measurements of cross sections using an a priori knowledge of the incoming neutrino energy.
